Asymptotic Estimates in Information Theory with Non-Vanishing Error Probabilities

This monograph presents a unified treatment of single- and multi-user problems in Shannon's information theory where we depart from the requirement that the error probability decays asymptotically in the blocklength. Instead, the error probabilities for various problems are bounded above by a non-vanishing constant and the spotlight is shone on achievable coding rates as functions of the growing blocklengths. This represents the study of asymptotic estimates with non-vanishing error probabilities. In Part I, after reviewing the fundamentals of information theory, we discuss Strassen's seminal result for binary hypothesis testing where the type-I error probability is non-vanishing and the rate of decay of the type-II error probability with growing number of independent observations is characterized. In Part II, we use this basic hypothesis testing result to develop second- and sometimes, even third-order asymptotic expansions for point-to-point communication. Finally in Part III, we consider network information theory problems for which the second-order asymptotics are known. These problems include some classes of channels with random state, the multiple-encoder distributed lossless source coding (Slepian-Wolf) problem and special cases of the Gaussian interference and multiple-access channels. Finally, we discuss avenues for further research.

==> common_pic.tex <==
\put(0, 10){\vector(1, 0){110}}
\put(10, 0){\vector(0,1){110}}
\put(50, 30){\line(1, 0){55}}
\put(30, 50){\line(0,1){55}}
\put(50, 30){\line(-1, 1){20}}
\put(110,8){ $R_1$}
\put(-6, 105){ $R_2$}
\multiput(10,50)(4,0){5}{\line(1,0){2}}
\put(-5, 50){$H_2$}
\put(-10, 30){$H_{2|1}$}
\multiput(10,30)(4,0){10}{\line(1,0){2}}
\multiput(50,10)(0,4){5}{\line(0,1){2}}
\multiput(30,10)(0,4){10}{\line(0,1){2}}
\put(50, 0){$H_1$}
\put(25, 0){$H_{1|2}$}
  \thicklines
\qbezier(40,70)(38,38)(70,40)
\put(70, 40){\line(1, 0){35}}
\put(40, 70){\line(0, 1){35}}
\put(60, 70){$\scR^*_{\mathrm{SW}}(n,\epsilon)$}
%\put(70, 80){\footnotesize $\tilde{\scR}_{\mathrm{SW}} (n,\epsilon)$}
%\put(95, 22){\footnotesize $\scB^*_{\mathrm{SW}} $}
  \thinlines

==> diag_slice.tex <==
\begin{picture}(115, 115)
\input{common_pic}

\put(60, 70){\vector(-1,-1){25}}
%\put(56, 56){\footnotesize $\vec{\bd}$}
%\put(10, 82){\line(1,-1){61}}
%\put(70, 14){\footnotesize $\scL_c$}
%\put(3, 81){\footnotesize $c$}
\multiput(35,45)(4,0){8}{\line(1,0){2}}
\qbezier(50,60)(55,55)(55,45)
\put(57,50){\footnotesize $\theta$}
\end{picture}

==> disp_slices.tex <==
\section{Dispersion Along Slices of the $(n,\epsilon)$-Rate Regions} \label{sec:dispSlice}

While we have a single-letter characterization of the $(n,\epsilon)$-optimal rate region for SW coding and inner bounds for the   $(n,\epsilon)$-capacity regions for the DM-MAC and DM-ABC problems,  it is instructive to study the behavior along certain ``slices'' of the region. We would also like to compute, if possible,  the dispersion (second-order coding rate) as a rate pair converges to a particular point  on the boundaries of the asymptotic regions.  To be concrete, we will focus solely on the SW setting (Theorem~\ref{thm:orr}) but we note that similar conclusions can be made for the inner bound to the $(n,\epsilon)$-capacity region for the DM-MAC for fixed input distributions (Theorem~\ref{thm:mac}).   We start by defining  the set
\begin{equation}
\tilde{\scR}_{\mathrm{SW}} (n,\epsilon) := \left\{  (R_1, R_2)  \in \bbR^2: \bR  \in \bH + \frac{1}{\sqrt{n}}\scS(\bV,\epsilon)\right\}.  \label{eqn:tildeR}
\end{equation}
Observe that $\tilde{\scR}_{\mathrm{SW}}(n,\epsilon)$ is  essentially the same as   $\scR^*_{\mathrm{SW}}(n,\epsilon)$ but the former  ignores  the $O(\frac{\log n}{n})$ terms in the inner and outer bounds of Theorem~\ref{thm:orr}.  The set in \eqref{eqn:tildeR} is shown in Fig.~\ref{fig:slices}. Assume for the rest of this section that the entropy dispersion matrix $\bV (p_{X_1, X_2}) \succ 0$ so in particular, conditioning strictly reduces entropy, i.e., $H(X_1|X_2)<H(X_1)$. This ensures that the SW region is non-degenerate.

\begin{figure}
\centering
\begin{tabular}{ccc}
\input{hor_slice} &  \hspace{.35in}
\input{diag_slice} &  \hspace{.35in}
\input{cor_slice} \\
(a) &  \hspace{.35in} (b)&  \hspace{.35in} (c) 
\end{tabular}
\caption{Plots of the approximation to the $(n,\epsilon)$-optimal rate region $\tilde{\scR}_{\mathrm{SW}} (n,\epsilon)$ defined in \eqref{eqn:tildeR} and the asymptotic SW region in \eqref{eqn:sw_reg} whose boundary is indicated by $\scB_{\mathrm{SW}}^*$. We use the simplified notation $H_1:= H(X_1), H_2:= H(X_2), H_{1|2}:= H(X_1|X_2)$,  $H_{2|1}:= H(X_2|X_1)$ and $H_{1,2}=H(X_1, X_2)$. The directions of approach   are indicated by the arrows in the different subplots. In subplot (a), we approach the vertical boundary. The dispersion $F$ is given in~\eqref{eqn:subplota}. In subplot (b), we approach the sum rate boundary. The dispersion  $F$ is given in~\eqref{eqn:subplotb}. In subplot (c), we approach the corner point $(H_1, H_{2|1})$. The dispersion $F$ is given  implicitly in~\eqref{eqn:subplotc}. The point  $(R_1(n,\epsilon), R_2(n,\epsilon))$ (defined in \eqref{eqn:R1ne} and~\eqref{eqn:R2ne}) and the point target point $(R_1^*, R_2^*)$ are also indicated in (c). } \label{fig:slices}
\end{figure}

As we see in Fig.~\ref{fig:slices}, we can approach a point on the asymptotic SW boundary, denoted as $\scB^*_{\mathrm{SW}}$, from a number of different directions. We formalize this as follows: Let $\theta$ be an \emph{angle of approach} towards a point $(R_1^*, R_2^*)$ lying on the SW boundary $\scB^*_{\mathrm{SW}}$. We use a single {\em dispersion-like} quantity  $F=F(\theta,\epsilon)$ to parametrize  the approach of a pair of rates towards $(R_1^*, R_2^*)$. More precisely, define 
\begin{align}
R_1(n,\epsilon)&:= R_1^* + \sqrt{\frac{F}{n}} (\cos \theta) \, \rmQ^{-1}(\epsilon)  \label{eqn:R1ne} \\
R_2(n,\epsilon)&:= R_2^* + \sqrt{\frac{F}{n}} (\sin \theta) \, \rmQ^{-1}(\epsilon) .\label{eqn:R2ne}  
\end{align}
In other words,  $(R_1(n,\epsilon), R_2(n,\epsilon))$  is a rate pair on the boundary of the region $\tilde{\scR}_{\mathrm{SW}} (n,\epsilon)$ that approaches $(R_1^*, R_2^*)$ at a rate governed by the angle of approach $\theta$, the error probability in the form of the Gaussian approximation term  $\rmQ^{-1}(\epsilon)$, and the {\em effective dispersion} $F$. The following proposition leverages on Theorem~\ref{thm:orr} to  quantify the minimum  $F$ achieving $\epsilon$ probability of error  for various   $(R_1^*,R_2^*,\theta)$. To state our result cleanly, we define 
\begin{equation}
\Psi(\rho; x',y'):= \frac{1}{2\pi\sqrt{1-\rho^2}} \int_{x'}^{\infty}\int_{y'}^{\infty} \exp \left\{ -\frac{x^2-2\rho xy+y^2}{2(1-\rho^2)} \right\}\, \mathrm{d}y  \, \mathrm{d}x,   \label{eqn:Psi}
\end{equation}
as  the bivariate generalization of the $\rmQ$-function.  

\begin{proposition}[Dispersion Along Slices of $(n,\epsilon)$-SW Region] \label{prop:slices}
Let   $\tau_n$ be an exponentially decaying sequence\footnote{The sequence $\{\tau_n\}_{n=1}^{\infty}$ is {\em exponentially decaying} if $\limsup_{n\to\infty}\frac{1}{n}\log \tau_n<0$.}    that may change from line to line. There are five different cases. First, assume that $(R_1^*,R_2^*)$ is not a corner point. In particular, let $R_1^* = H(X_1|X_2) $ and  let $R_2^*>H(X_2)$ (vertical boundary). Then,
\begin{equation}
F= \frac{[\bV]_{1,1}}{ \cos^2 \theta     } + \tau_n. \label{eqn:subplota}
\end{equation}
Similarly if $R_2^*=H(X_2|X_1)$ and   $R_1^*>H(X_1)$ (horizontal boundary)  then,
\begin{equation}
F= \frac{[\bV]_{2,2}}{ \sin^2 \theta     } +\tau_n. \label{eqn:hori}
\end{equation}
Similarly if $R_1^*+R_2^*=H(X_1, X_2)$, $R_1^*>H(X_1|X_2)$ and  $R_2^*>H(X_2|X_1)$  (sum rate boundary) then,
\begin{equation}
F= \frac{[\bV]_{3,3}}{  (\cos \theta+\sin \theta)^2 }+\tau_n. \label{eqn:subplotb}
\end{equation}
Now assume that   $(R_1^*,R_2^*)$ is   a corner point. In particular, let   $R_1^*= H(X_1|X_2) $ and $R_2^* = H(X_2)$. Then $F$ is the solution to 
\begin{equation}
\Psi \left(\rho_{1,3};-\sqrt{\frac{F}{[\bV]_{1,1}}} \, (\cos\theta)\, \rmQ^{-1}(\epsilon), -\sqrt{\frac{F}{[\bV]_{3,3}}} \, (\cos\theta+\sin\theta)\, \rmQ^{-1}(\epsilon) \right) = 1-\epsilon+\tau_n, \label{eqn:corner_pt}
\end{equation}
where $\rho_{1,3}:=[\bV]_{1,3}/\sqrt{[\bV]_{1,1}[\bV]_{3,3}}$ is the correlation coefficient of  the random variables $-\log p_{X_1|X_2}(X_1|X_2)$ and  $-\log p_{X_1,X_2}(X_1, X_2)$.   % and  the functions $g_{\mathrm{c}}$ and $g_{\mathrm{sc}}$ are defined as
%\begin{align}
%g_{\mathrm{c}}(F,v) & := -\sqrt{\frac{F}{v}} \, (\cos\theta)\, \rmQ^{-1}(\epsilon) \label{eqn:gc} \\*
%g_{\mathrm{sc}}(F,v) & :=-\sqrt{\frac{F}{v}} \, (\cos\theta+\sin\theta)\, \rmQ^{-1}(\epsilon) \label{eqn:gsc} .
%\end{align}
Finally, if $R_1^*= H(X_1 ) $ and $R_2^* = H(X_2|X_1)$, then $F$ is the solution to 
\begin{equation}
\Psi \left(\rho_{2,3};-\sqrt{\frac{F}{[\bV]_{2,2}}} \, (\sin\theta)\, \rmQ^{-1}(\epsilon), -\sqrt{\frac{F}{[\bV]_{3,3}}} \, (\cos\theta+\sin\theta)\, \rmQ^{-1}(\epsilon) \right) = 1-\epsilon+\tau_n, \label{eqn:subplotc}
\end{equation}
%where the function  $g_{\mathrm{s}}$ is defined as 
%\begin{equation}
%g_{\mathrm{s}}(F,v) :=-\sqrt{\frac{F}{v}} \, (\sin\theta)\, \rmQ^{-1}(\epsilon)\label{eqn:gs}
%\end{equation}
\end{proposition}
This proposition is proved in Appendix~\ref{app:slice}.  Intuitively, for \eqref{eqn:subplota}--\eqref{eqn:subplotb}, two (our of three) of probabilities of the constituent events  that comprise $\{\bZ\le\sqrt{n}(\bR(n,\epsilon)-\bH)\}$ decay exponentially fast since we are operating ``far from'' the corresponding constraints. For \eqref{eqn:corner_pt} and \eqref{eqn:subplotc}, only one such probability   decays exponentially fast so two constraints are still active.
 
The interpretations of~\eqref{eqn:subplota} to~\eqref{eqn:subplotb} are fairly clear. The dispersion-like quantity $F$  depends on  the angle of approach to the boundary $\theta$ and the corresponding entry in the diagonal of the entropy dispersion matrix. So for example, if we are approaching the vertical boundary as in Fig.~\ref{fig:slices}(a), then  substituting  the result~\eqref{eqn:subplota} into \eqref{eqn:R1ne}  and \eqref{eqn:R2ne}  yields
\begin{align}
R_1(n,\epsilon)&=H(X_1|X_2)+\sqrt{\frac{[\bV]_{1,1} }{n}}\, \rmQ^{-1}(\epsilon) +\tau_n \label{eqn:rate1}\\
R_2(n,\epsilon)&=H(X_2 )+\sqrt{\frac{[\bV]_{1,1} }{n}}\,(\tan\theta)\, \rmQ^{-1}(\epsilon)+\tau_n,
\end{align}
which is simply a scalar dispersion result. If instead we are approaching either one of the corner points, say $( H(X_1), H(X_2|X_1))$, at an angle $\theta$ as in Fig.~\ref{fig:slices}(c), then the situation is much more complicated and $F$ is given as in \eqref{eqn:subplotc}. Intuitively, this is because there are several forces at play ---   the contribution from the marginal dispersion $[\bV]_{2,2}$, the contribution from the  sum rate dispersion $[\bV]_{3,3}$ and also their correlation coefficient $\rho_{2,3}$. These interact to give an effective dispersion that can only be expressed implicitly in the form shown in \eqref{eqn:subplotc}. Note that now $F$ depends   on the angle of approach and the correlation  coefficient of  $-\log p_{X_2|X_1}(X_2|X_1)$ and $-\log p_{X_1, X_2}(X_1, X_2)$ namely $\rho_{2,3}$. Interestingly, $F$ {\em also} depends on $\epsilon$ unlike the corresponding scalar results in \eqref{eqn:subplota}--\eqref{eqn:subplotb}. We will verify this numerically in Section~\ref{sec:theta}.

We now interpret Proposition~\ref{prop:slices} operationally from the perspective of another source coding problem. Consider the $(n,\epsilon)$-region for lossless source coding with side information  at encoders and decoder (SI-ED), also known as {\em cooperative} source coding.  Specifically, first consider the problem of source coding $X_1$ with $X_2$ available as (full non-coded) side information at the encoder and the decoder. Second, we swap the roles of $X_1$ and $X_2$. Third, we consider a source coding problem for the pair  $(X_1,X_2)$. Up to   $O(\frac{\log n}{n})$ terms, this region  $\scR^*_{\mathrm{SI-ED}}(n,\epsilon) \subset\bbR^2$ is the set of rate pairs $(R_1, R_2)$ satisfying the three scalar constraints
\begin{align}
R_1&\ge H(X_1|X_2)+\sqrt{\frac{[\bV]_{1,1}}{n}}\, \rmQ^{-1}(\epsilon)  \nn\\*
R_2&\ge H(X_2|X_1)+\sqrt{\frac{[\bV]_{2,2}}{n}}\, \rmQ^{-1}(\epsilon)  \nn\\*
R_1+R_2&\ge H(X_1,X_2)+\sqrt{\frac{[\bV]_{3,3}}{n}}\, \rmQ^{-1}(\epsilon)   . \label{eqn:sied} 
\end{align}
The three {\em decoupled} constraints in \eqref{eqn:sied} represent three single-user simplifications of the problem and therefore are three crude outer bounds to $\scR^*_{\mathrm{SW}}(n,\epsilon)$. The first two inequalities characterizing the region in \eqref{eqn:sied} can be derived in a straightforward manner using a side information (conditional) version of Strassen's original result~\cite{strassen} for hypothesis testing. The last inequality is simply one of Strassen's original results on source coding. Also see Problem 1.1.8 in  Csisz\'{a}r and   K\"{o}rner~\cite{Csi97} and Theorem 1 in Kontoyiannis~\cite{Kot97}. Our Theorem \ref{thm:orr} says that this {\em scalar} perspective on dispersion is insufficient for multi-user problems. However, away from corner points, Proposition \ref{prop:slices} asserts that SW coding is very close to the boundaries of the $(n,\epsilon)$-SI-ED region    $\scR^*_{\mathrm{SI-ED}}(n,\epsilon)$. For example, we see from \eqref{eqn:rate1}, which is consequence of \eqref{eqn:subplota}, that the  rate $R_1$   for SW coding and SI-ED coding are the same up to an exponentially decaying term,  which is subsumed by the Berry-Ess\`{e}en residual term of order $O(\frac{\log n}{n})$. Thus, SW coding and SI-ED coding are essentially the same away from the corner points.  At the corner points, the story is   different and more complicated as we observed in~\eqref{eqn:corner_pt} and~\eqref{eqn:subplotc}.% We study this numerically in the following section. 
